Measurement and Calibration of Noise Bias in Weak Lensing Galaxy Shape Estimation

Weak gravitational lensing has the potential to constrain cosmological parameters to high precision. However, as shown by the Shear TEsting Programmes (STEP) and GRavitational lEnsing Accuracy Testing (GREAT) Challenges, measuring galaxy shears is a nontrivial task: various methods introduce different systematic biases which have to be accounted for. We investigate how pixel noise on the image affects the bias on shear estimates from a Maximum-Likelihood forward model-fitting approach using a sum of co-elliptical S\'{e}rsic profiles, in complement to the theoretical approach of an an associated paper. We evaluate the bias using a simple but realistic galaxy model and find that the effects of noise alone can cause biases of order 1-10% on measured shears, which is significant for current and future lensing surveys. We evaluate a simulation-based calibration method to create a bias model as a function of galaxy properties and observing conditions. This model is then used to correct the simulated measurements. We demonstrate that this method can effectively reduce noise bias so that shear measurement reaches the level of accuracy required for estimating cosmic shear in upcoming lensing surveys.

==> nbc_paper_methods.tex <==
\section{Method of measuring the pixel noise bias}
\label{sec:Methods}

%S1 [need an orientation paragraph between section and subsection. In this case though I think we don't need the subsection]
%S1 \subsection{Approach}

In this paper we demonstrate a method to obtain an unbiased ellipticity estimate for a fiducial galaxy. We believe it can be easily extended to the full parameter space covered in galaxies in weak lensing survey. However, increasing the number of parameters used in the model will increase the difficulty of this.

We propose a following procedure
\begin{enumerate}
\item {Measure the noise bias for the fiducial galaxy and it's neighbours in galaxy and image parameter space}
\item {Apply the calibration based on measured bias to the noisy MLE estimates}
\end{enumerate}

For a fiducial galaxy, pixel noise will cause the MLE to be scattered around the truth with some unknown, often skewed distribution. The variance of this distribution will depend strongly on SNR. As we apply the correction to the noisy esimates, we choose the points in galaxy and image parameters based on the variance of the ML esimates for the fiducial galaxy at the SNR of 10. For these parameters we measure the bias and use those interpolate to any point in covered parameter space. Measurement of the bias for a single parameter set is compuationally very expensive and it is intractable to do it for all their combinations. Therefore we treat the infulence of each parameter on the bias as independent and evaluate the bias for a fiducial parameter set and deviation in one parameter at a time. We factorise the bias funtion as 
{\bf this will probably change}\newline
\begin{equation}
b(\vec{\theta}) = \frac{1}{Z}\prod_i b([\theta^{fid}_1, \theta^{fid}_2, \dots , \theta_i, \dots , \theta^{fid}_n ]) 
\label{eqn:BFactors}
\end{equation}
where $Z$ is a normalisation factor. We show that this approximation is satisfactory to desired accuracy. The choise of the number of points depents of how smoothly the bias function changes in examined regime; we find that for most parameters 3 points (including fiducial) is enough to perform accurate interpolation. For SNR more parameter values were measured. The number of points can be increased at the expense of additional compuation time.  

This approach is in fact very similar to the one used in GREAT08 and GREAT10, where fiducial model and one-parameter deviations from it were used. 

The calibration is applied to noisy estimates, therefore each estimate will not be corrected exactly. Despite that, this calibration procedure is effective to a level sufficient for upcoming galaxy surveys, as it will be shown in Section \ref{sec:Application}.

%S1 - moved this subsection to end of section 2 to be more conventional
%S1 \subsection{Chosen parameters and simulation details}



